Practical Sketching-Based Randomized Tensor Ring Decomposition

Based on sketching techniques, we propose two randomized algorithms for tensor ring (TR) decomposition. Specifically, by defining new tensor products and investigating their properties, we apply the Kronecker sub-sampled randomized Fourier transform and TensorSketch to the alternating least squares problems derived from the minimization problem of TR decomposition to devise the randomized algorithms. From the former, we find an algorithmic framework based on random projection for randomized TR decomposition. Theoretical results on sketch size and complexity analyses for the two algorithms are provided. We compare our proposals with the state-of-the-art method using both synthetic and real data. Numerical results show that they have quite decent performance in accuracy and computing time

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
